Generative Model for Models: Rapid DNN Customization for Diverse Tasks and Resource Constraints

Unlike cloud-based deep learning models that are often large and uniform, edge-deployed models usually demand customization for domain-specific tasks and resource-limited environments. Such customization processes can be costly and time-consuming due to the diversity of edge scenarios and the training load for each scenario. Although various approaches have been proposed for rapid resource-oriented customization and task-oriented customization respectively, achieving both of them at the same time is challenging. Drawing inspiration from the generative AI and the modular composability of neural networks, we introduce NN-Factory, an one-for-all framework to generate customized lightweight models for diverse edge scenarios. The key idea is to use a generative model to directly produce the customized models, instead of training them. The main components of NN-Factory include a modular supernet with pretrained modules that can be conditionally activated to accomplish different tasks and a generative module assembler that manipulate the modules according to task and sparsity requirements. Given an edge scenario, NN-Factory can efficiently customize a compact model specialized in the edge task while satisfying the edge resource constraints by searching for the optimal strategy to assemble the modules. Based on experiments on image classification and object detection tasks with different edge devices, NN-Factory is able to generate high-quality task- and resource-specific models within few seconds, faster than conventional model customization approaches by orders of magnitude.

==> tex/discussion.tex <==
\section{Discussion}\label{sec:discussion}

There may be some issues with \name that warrant further discussion.Firstly, we should address the requirements within the task space.Utilizing one-hot encoding to bestow semantic information to each bit proves to be highly effective for encoding tasks,however, this approach demands an adequate number of tasks to enable \name to comprehend the semantic representation associated with each bit.Additionally, as the number of semantic units decomposed increases, the required quantity of tasks for training also grows.


==> tex/related_work.tex <==
\section{Related Work}\label{sec:related_work}


